Latent Gaussian Model Boosting

Latent Gaussian models and boosting are widely used techniques in statistics and machine learning. Tree-boosting shows excellent prediction accuracy on many data sets, but potential drawbacks are that it assumes conditional independence of samples, produces discontinuous predictions for, e.g., spatial data, and it can have difficulty with high-cardinality categorical variables. Latent Gaussian models, such as Gaussian process and grouped random effects models, are flexible prior models which explicitly model dependence among samples and which allow for efficient learning of predictor functions and for making probabilistic predictions. However, existing latent Gaussian models usually assume either a zero or a linear prior mean function which can be an unrealistic assumption. This article introduces a novel approach that combines boosting and latent Gaussian models to remedy the above-mentioned drawbacks and to leverage the advantages of both techniques. We obtain increased prediction accuracy compared to existing approaches in both simulated and real-world data experiments.

==> results_poverty.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Mon Dec 20 07:55:33 2021
\begin{table}[ht!]
\centering
\begingroup\footnotesize
\begin{tabular}{rllll}
  \hline
\hline
  & LaGaBoost & LinearME & LogitBoost & mboost \\ 
  \hline
Error & \bf{0.2792} & 0.2848 & 0.3239 & 0.3197 \\ 
  AUC & \bf{0.7318} & 0.7313 & 0.7001 & 0.7028 \\ 
  Log\_loss & \bf{0.5789} & 0.5878 & 0.6013 & 0.6081 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Comparison of predictive accuracy for the poverty data.} 
\label{results_poverty}
\end{table}


==> results_poverty_caption_top.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Mon Dec 20 07:55:33 2021
\begin{table*}[ht!]
\centering
\caption{Comparison of predictive accuracy for the poverty data.} 
\label{results_poverty}
\begingroup\footnotesize
\begin{tabular}{rllll}
  \hline
\hline
  & LaGaBoost & LinearME & LogitBoost & mboost \\ 
  \hline
Error & \bf{0.2792} & 0.2848 & 0.3239 & 0.3197 \\ 
  AUC & \bf{0.7318} & 0.7313 & 0.7001 & 0.7028 \\ 
  Log\_loss & \bf{0.5789} & 0.5878 & 0.6013 & 0.6081 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\end{table*}


==> results_species.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Mon Dec 20 07:55:33 2021
\begin{table}[ht!]
\centering
\begingroup\footnotesize
\begin{tabular}{rllll}
  \hline
\hline
  & LaGaBoost & LinearGP & LogitBoost & mboost \\ 
  \hline
Error & \bf{0.2365} & 0.3003 & 0.2717 & 0.2728 \\ 
  AUC & \bf{0.7383} & 0.7061 & 0.683 & 0.635 \\ 
  Log\_loss & \bf{0.4933} & 0.5625 & 0.527 & 0.5662 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\caption{Comparison of predictive accuracy for the species data.} 
\label{results_species}
\end{table}


==> results_species_caption_top.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Mon Dec 20 07:55:33 2021
\begin{table*}[ht!]
\centering
\caption{Comparison of predictive accuracy for the species data.} 
\label{results_species}
\begingroup\footnotesize
\begin{tabular}{rllll}
  \hline
\hline
  & LaGaBoost & LinearGP & LogitBoost & mboost \\ 
  \hline
Error & \bf{0.2365} & 0.3003 & 0.2717 & 0.2728 \\ 
  AUC & \bf{0.7383} & 0.7061 & 0.683 & 0.635 \\ 
  Log\_loss & \bf{0.4933} & 0.5625 & 0.527 & 0.5662 \\ 
   \hline
\hline
\end{tabular}
\endgroup
\end{table*}

